Noisy Parallel Data Alignment

An ongoing challenge in current natural language processing is how its major advancements tend to disproportionately favor resource-rich languages, leaving a significant number of under-resourced languages behind. Due to the lack of resources required to train and evaluate models, most modern language technologies are either nonexistent or unreliable to process endangered, local, and non-standardized languages. Optical character recognition (OCR) is often used to convert endangered language documents into machine-readable data. However, such OCR output is typically noisy, and most word alignment models are not built to work under such noisy conditions. In this work, we study the existing word-level alignment models under noisy settings and aim to make them more robust to noisy data. Our noise simulation and structural biasing method, tested on multiple language pairs, manages to reduce the alignment error rate on a state-of-the-art neural-based alignment model up to 59.6%.

==> stash.tex <==
\iffalse
\begin{table*}[h!]
\centering
\begin{tabular}{@{ }l@{ }c@{ }c@{ }c@{ }c|c@{ }c@{ }c@{ }c@{ }} 
 \toprule
 Augm. Data & \multicolumn{4}{c|}{Unsupervised-Finetune} & \multicolumn{4}{c}{Supervised-Finetune} \\
CER (WER) & \tiny Clean-Clean& \tiny Clean-Synth& \tiny Synth-Clean& \tiny Synth-Synth & \tiny Clean-Clean& \tiny Clean-Synth& \tiny Synth-Clean& \tiny Synth-Synth\\
\midrule
%\textsc{w/o fine. (original)}& 5.6& 39.2& 40.5& 53.6 \\
\textit{Skyline}\\
\textsc{ 7.4-4.8 (72-71)} & 4.3&37& 34.4& 46.9  &6.8& 31.1& 30& 40.3  \\
\midrule
\textit{Unified}\\
\textsc{2-2 (32-29)} & 4.1 & 37.5 & 35.1 & 48.4 & \textbf{5.1}& 33.3& 30.1& 41.8\\
\textsc{5-5 (55-52)} & & & &  &  7.4& \textbf{30.4}& \textbf{29.8}& \textbf{40}\\
\textsc{10-10 (72-71)} & 4.5 & 36.8 & 34.5 & 46.8 & 32.8 & 36.2& 47.7 & 47.3\\
\textsc{mixed(55-54)} & 5.4 & 37.3 & 35.3 & 47.7  &  5.5& 39.6& 39.8& 54.2\\ 
\midrule

\textit{Random}\\
\textsc{1.6-2.1(27.8-29.6)} & \textbf{4.0} & 37.6 & 35 & 48.4 &  6.2& 31.6& 30.6& 41.9\\
\textsc{4.1-5.1(49.6-52.5} & 4.3& 37& 34.7& 47.2 &  7.7& 29.8& 30.1& \textbf{40.2}\\
\textsc{8.1-9.6(66.9-69.5)} & 4.5& 37.1& \textbf{34.3}& \textbf{46.7}& 31.3 & 36.2& 46.3 & 46.9\\
\textsc{mixed(47.9-50)} & 4.2& \textbf{37}& 34.6& 47.2 &  \textbf{5.6}& \textbf{29.3}& \textbf{29.7}& 40.4\\
\bottomrule

\end{tabular}
\caption{AER comparison for varying CER in 100K English-French dataset under \textbf{unsupervised} setting. Overall, the model performance is close to the baseline. \rz{might need to rephrase depending on keeping 'random' CER or not}}
\label{table:UnsupervisedCER}
\end{table*}

\begin{table*}[h!]
\centering
\begin{tabular}{c c c c c} 
 \toprule
En-Fr CER (WER) & Clean-Clean& Clean-Synthetic& Synthetic-Clean& Synthetic-Synthetic\\
\midrule
% \textsc{w/o fine. (original)}& 5.6& 39.2& 40.5& 53.6 \\
\textit{Skyline}\\
\textsc{ 7.4-4.8 (72-71)} &6.8& 31.1& 30& 40.3  \\
\hline
\textit{Unified}\\
\textsc{2-2 (32-29)} & \textbf{5.1}& 33.3& 30.1& 41.8\\
\textsc{5-5 (55-52)} &  7.4& \textbf{30.4}& \textbf{29.8}& \textbf{40}\\
\textsc{10-10 (72-71)} & 32.8 & 36.2& 47.7 & 47.3\\
\textsc{mixed(55-54)} &  5.5& 39.6& 39.8& 54.2\\
\hline
\textit{Random} \rz{keeping them?} \\
\textsc{1.6-2.1(27.8-29.6)} &  6.2& 31.6& 30.6& 41.9\\
\textsc{4.1-5.1(49.6-52.5} &  7.7& 29.8& 30.1& \textbf{40.2}\\
\textsc{8.1-9.6(66.9-69.5)} & 31.3 & 36.2& 46.3 & 46.9\\
\textsc{mixed(47.9-50)} &  \textbf{5.6}& \textbf{29.3}& \textbf{29.7}& 40.4\\
\bottomrule

\end{tabular}
\caption{AER comparison for \textbf{supervised} finetuning with various CER for 100K English-French dataset. Clean test set breaks with 10 CER for both side of the language pairs \rz{might need to rephrase depending on keeping 'random' CER or not}}
\label{table:supervisedCER}
\vspace{-1em}
\end{table*}
\fi


